Preserving Generalization of Language models in Few-shot Continual Relation Extraction

Few-shot Continual Relations Extraction (FCRE) is an emerging and dynamic area of study where models can sequentially integrate knowledge from new relations with limited labeled data while circumventing catastrophic forgetting and preserving prior knowledge from pre-trained backbones. In this work, we introduce a novel method that leverages often-discarded language model heads. By employing these components via a mutual information maximization strategy, our approach helps maintain prior knowledge from the pre-trained backbone and strategically aligns the primary classification head, thereby enhancing model performance. Furthermore, we explore the potential of Large Language Models (LLMs), renowned for their wealth of knowledge, in addressing FCRE challenges. Our comprehensive experimental results underscore the efficacy of the proposed method and offer valuable insights for future work.

==> secs/9-motivation.tex <==
\subsubsection{Motivation}

% Starting from why consider using pretrained-LLM heads: situation, context..
Pretrained large language models \textbf{[CITE]} are revolutionizing the way we approach language understanding and generation. Their extensive training on vast amounts of data equips them with unparalleled generalizability, making them invaluable for various downstream tasks. While traditional LLMs with autoregressive behavior excel in text generation, recent discoveries \textbf{[CITE]} have shed light on their limitations in labeled supervised tasks. Therefore, researchers often only take advantage of the pre-trained backbone and ignore the head part of the LLM \textbf{[CITE}]. 

However, we firmly believe that the pre-trained LLM heads can significantly enhance the model performance if used strategically. Thus, it is imperative to reconsider how we harness the potential of these large models by examining their entire architecture rather than solely focusing on the pre-trained backbones. Embracing this comprehensive approach will unlock even greater possibilities for innovation and problem-solving.

On the one hand, in recent FCRE work \textbf{[CITE]}, when learning a classification head from scratch across multiple tasks, the emphasis is often on discriminative features derived from sparse data streams and memory buffers. This focus can not only lead the model to rapidly forget previous knowledge but also make predictions that lack comprehensiveness. On the other hand, pre-trained language model (LLM) heads are inherently trained to make predictions on a vast vocabulary set containing highly generalized and meaningful information. Leveraging this knowledge will complement our primary classifier, aiding the model in capturing information more effectively and thus helping to address two complex problems: catastrophic forgetting and overfitting in FCRE. Therefore, inspired by \textbf{[OCM]}, we aim at using MMI loss to effectively distill knowledge holistically from an LLM head to our main classifier. In particular, we propose to maximize Mutual Information between logit vectors from the LLM head and the conventional main classifier. 

Moreover, to investigate the role of Large Language Models (LLMs) and provide valuable insights to the research community, we are assessing the use of pre-trained LLMs for Few-Shot Continual Relation Extraction problems. Our research question is: \textit{Can LLMs, equipped with large architectures and trained on extensive data, effectively address FCRE challenges?} Specifically, can the general knowledge embedded in these models help mitigate the two primary concerns of FCRE: catastrophic forgetting and overfitting, which is due to data sparsity? Furthermore, will the results obtained demonstrate the effectiveness of the proposed new strategy?
